Addressing target shift in zero-shot learning using grouped adversarial learning

Zero-shot learning (ZSL) algorithms typically work by exploiting attribute correlations to be able to make predictions in unseen classes. However, these correlations do not remain intact at test time in most practical settings and the resulting change in these correlations lead to adverse effects on zero-shot learning performance. In this paper, we present a new paradigm for ZSL that: (i) utilizes the class-attribute mapping of unseen classes to estimate the change in target distribution (target shift), and (ii) propose a novel technique called grouped Adversarial Learning (gAL) to reduce negative effects of this shift. Our approach is widely applicable for several existing ZSL algorithms, including those with implicit attribute predictions. We apply the proposed technique ($g$AL) on three popular ZSL algorithms: ALE, SJE, and DEVISE, and show performance improvements on 4 popular ZSL datasets: AwA2, aPY, CUB and SUN. We obtain SOTA results on SUN and aPY datasets and achieve comparable results on AwA2.

==> comparewithcvpr.tex <==
A version of this paper was submitted to CVPR 2020.

Summary of reviews:
- The major complaint from the reviewers is the lack of SOTA level performance scores on benchmark datasets. The reviewers also questioned sufficient reasons for gAL's performance.  There were also questions on why we only applied gAL technique on just one ZSL algorithm and which all ZSL algorithms can this technique be extended to.

Changes made:
- We now extended gAL algorithm to four ZSL methods and clearly define the conditions for any other ZSL algorithm to which it may be applied. The additional approaches now helped us achieve SOTA on 2 out of the 4 benchmark datasets, along with close to SOTA in the third dataset.
- We greatly improve the articulation of the paper, providing several additional citations and views to the problem from new directions.
- We now have an explanation for the question asked by 2 reviewers: "why gAL works?". More intuitions on our contributions are added.
- We are now submitting a modular, extendable Python+pytorch code in supplementary with the new experimental benchmark.
